EdgeOAR: Real-time Online Action Recognition On Edge Devices

This paper addresses the challenges of Online Action Recognition (OAR), a framework that involves instantaneous analysis and classification of behaviors in video streams. OAR must operate under stringent latency constraints, making it an indispensable component for real-time feedback for edge computing. Existing methods, which typically rely on the processing of entire video clips, fall short in scenarios requiring immediate recognition. To address this, we designed EdgeOAR, a novel framework specifically designed for OAR on edge devices. EdgeOAR includes the Early Exit-oriented Task-specific Feature Enhancement Module (TFEM), which comprises lightweight submodules to optimize features in both temporal and spatial dimensions. We design an iterative training method to enable TFEM learning features from the beginning of the video. Additionally, EdgeOAR includes an Inverse Information Entropy (IIE) and Modality Consistency (MC)-driven fusion module to fuse features and make better exit decisions. This design overcomes the two main challenges: robust modeling of spatio-temporal action representations with limited initial frames in online video streams and balancing accuracy and efficiency on resource-constrained edge devices. Experiments show that on the UCF-101 dataset, our method EdgeOAR reduces latency by 99.23% and energy consumption by 99.28% compared to state-of-the-art (SOTA) method. And achieves an adequate accuracy on edge devices.

==> acknowledgments.tex <==
\section{Acknowledgments}
% 罗威、孙旺、何榜文、张德宇*、张昊、章晋睿、张熙铖、贾富程、张尧学
We thank Wang Sun and Bangwen He for they help on the experiments. \deyu{add Wang and Bangwen as co-authors}

==> discussion.tex <==
\section{Discussion}
\label{s.discussion}
\luov{Need to modify}
\textbf{Generality of \sysname.} 
\sysname represents an innovative system capable of achieving real-time instance segmentation on mobile devices. It leverages a contour-based segmentation method, utilizing MBs information from mobile device H.265, enabling rapid acquisition of contours close to the object edges, thus providing a robust starting point for subsequent contour deformation. Given the typically robust computational capabilities of CPUs in existing mobile phones, \sysname can be seamlessly deployed on these devices. Implemented using Java and C++, the system proves highly conducive to subsequent developmental references.


\textbf{Limitation and future work.} 
The current system exhibits several limitations that require addressing to enhance its performance and adaptability. Primarily, compared to pixel-domain images, MBs variations in consecutive frames still show significant differences. Although we have implemented spatiotemporal smoothing mechanisms, these tend to attenuate unique indications between different frames. Furthermore, the \sysname system has not sufficiently accounted for the impact of MB noise on contour initialization. At present, the system struggles to accurately locate object edges through small MBs. Therefore, acquiring a robust MBs map poses a challenge for the precise operation of \sysname. Thirdly, in the \sysname system, due to hardware encoding constraints of the DSP, the resulting H.265 video does not exhibit rectangular shapes (e.g., $32\times16$), leading to fewer hierarchical MBs, which complicates better shape representation. However, currently, using the smallest block size, $16\times16$, already meets the requirement.

To address these constraints, future work could involve integrating state-of-the-art algorithms and system optimizations to enhance the performance and adaptability of \sysname. For instance, potential approaches may include:
1) Proposing an improved contour initialization method that incorporates more compression domain information, such as MVs and residuals, based on certain changes in the visual content and MB map.
2) Developing a lightweight MBs smoothing solution that accounts for MBs shapes, thereby achieving improved MBs fusion outcomes.
